New Tricks for Estimating Gradients of Expectations

We introduce a family of pairwise stochastic gradient estimators for gradients of expectations, which are related to the log-derivative trick, but involve pairwise interactions between samples. The simplest example of our new estimator, dubbed the fundamental trick estimator, is shown to arise from either a) introducing and approximating an integral representation based on the fundamental theorem of calculus, or b) applying the reparameterisation trick to an implicit parameterisation under infinitesimal perturbation of the parameters. From the former perspective we generalise to a reproducing kernel Hilbert space representation, giving rise to a locality parameter in the pairwise interactions mentioned above, yielding our representer trick estimator. The resulting estimators are unbiased and shown to offer an independent component of useful information in comparison with the log-derivative estimator. We provide a further novel theoretical analysis which further characterises the variance reduction afforded by the new techniques. Promising analytical and numerical examples confirm the theory and intuitions behind the new estimators.

==> Autoref.tex <==
\usepackage{catoptions}
\makeatletter
\def\figureautorefname{figure}
\def\tableautorefname{table}
\def\Autoref#1{%
  \begingroup
  \edef\reserved@a{\cpttrimspaces{#1}}%
  \ifcsndefTF{r@#1}{%
    \xaftercsname{\expandafter\testreftype\@fourthoffive}
      {r@\reserved@a}.\\{#1}%
  }{%
    \ref{#1}%
  }%
  \endgroup
}
\def\testreftype#1.#2\\#3{%
  \ifcsndefTF{#1autorefname}{%
    \def\reserved@a##1##2\@nil{%
      \uppercase{\def\ref@name{##1}}%
      \csn@edef{#1autorefname}{\ref@name##2}%
      \autoref{#3}%
    }%
    \reserved@a#1\@nil
  }{%
    \autoref{#3}%
  }%
}
\makeatother

==> diversification.tex <==

\subsection{Motivation}

{\todo delete section}


\subsection{Usefulness of the Fundamental Trick in Convex Combination with the Log-Derivative}
\label{sec:diversification}

{\todo delete section}

==> diversification_ft.tex <==
\newcommand\sigmall{\hat\Sigma_\mathrm{ll}}
\newcommand\sigmafl{\hat\Sigma_\mathrm{fl}}
\begin{theorem}
\label{thm:divftld}
If both fundamental trick estimator $F_n$ of \eqref{eqn:logreparameterisationtrick:scalar:doublesum} and the log-derivative trick estimator $L_n$ of \eqref{eqn:logtrick:sum} have finite variance then in general $F_n$ diversifies $L_n$.
\end{theorem}
\begin{proof}
$L_n$ is unbiased \cite{reinforce}, and by \sref{Lemma}{lemma:unbiasedness} $F_n$ is an unbiased estimator of the same quantity. It is sufficient to check the $n=2$ case. Denote $L_2$ and $F_2$ by the subscripts l and f. The uncentered second moment $\sigmall$ of $F_2$ is the expectation w.r.t. $x, z\sim p(\cdot|\theta)$ of 
\begin{align}
& \Big( \frac{1}{2}\big(f(x)\nabla \log p(x|\theta)+f(z)\nabla \log p(z|\theta)\big) \Big)^2
\\ & ~= 
\frac{1}{4} \big( f(x)\nabla \log p(x|\theta)\big)^2
+
\frac{1}{4} \big(f(z)\nabla \log p(z|\theta)\big)^2
+
\frac{1}{2} f(x)\nabla \log p(x|\theta) f(z)\nabla \log p(z|\theta).~~~~~~
\label{eqn:crossll}
\end{align}
According to \sref{Lemma}{lemma:momentcondition} we need to check whether this equals $\sigmafl$, which is the expectation with respect to $x,z\sim p(\cdot|\theta)$ of the product of
\begin{align}
 & \frac{1}{2}
 \Big( 
 \frac{1}{p(x|\theta)}\mathbb I(z>x)f'(x) \nabla \log p(z|\theta) 
+ \frac{1}{p(z|\theta)}\mathbb I(x>z)f'(z) \nabla \log p(x|\theta) 
 \Big) 
 \end{align}
and
$
\frac{1}{2}
 \Big(
 f(x)\nabla \log p(x|\theta)+f(z)\nabla \log p(z|\theta)
 \Big).
$
But this expands to $1/4$ of the sum of four terms
\begin{align}
\label{eqn:crossa}
& \mathbb I(z>x)f'(x) \nabla \log p(z|\theta) 
f(x)\nabla \log p(x|\theta) / p(x|\theta)
\\ +~ &
\mathbb I(z>x)f'(x) \nabla \log p(z|\theta)
f(z)\nabla \log p(z|\theta) / p(x|\theta)
\\ +~ &
\mathbb I(x>z)f'(z) \nabla \log p(x|\theta)
f(x)\nabla \log p(x|\theta) / p(z|\theta)
\\ +~ &
\label{eqn:crossb}
\mathbb I(x>z)f'(z) \nabla \log p(x|\theta) 
f(z)\nabla \log p(z|\theta) / p(z|\theta).
\end{align}
The second and third of the four terms above correspond to the first and second terms on the r.h.s. of \eqref{eqn:crossll}. For example, the expectation w.r.t. $x$ of the second of the four terms is
\begin{align}
& \mathbb E_z\lsb \int_x \mathbb I(z>x)f'(x) \nabla \log p(z|\theta)f(z)\nabla \log p(z|\theta) \intd x\rsb 
\\ & ~~~ =
\label{eqn:ftmechanics}
\mathbb E_z\lsb f(z) \nabla \log p(z|\theta)f(z)\nabla \log p(z|\theta) \intd x\rsb
 = 
\mathbb E_z\lsb \lnb f(z) \nabla \log p(z|\theta) \rnb^2 \rsb,
\end{align}
which matches as claimed. The cross terms, however, (the first and fourth of the four terms) do not in general match those of \eqref{eqn:crossll}. Indeed, an analogous application of the fundamental theorem of calculus (as in \eqref{eqn:ftmechanics}) is inapplicable  because the variable involved appears in other factors. 
\end{proof}





==> ftexample_quadratic.tex <==

\subsection{Analytical Example}
\label{sec:ftexample}




\subparagraph{Setup} In the context of \eqref{eqn:goal}, consider $f(x)=x^2$ where $x,\theta\in\mathbb{R}$ and 
\begin{align}
p(x|\theta)
& = 
\frac{2}{\pi} \begin{cases}
1/(1+(x-\theta)^2) & \abs{x-\theta} \leq 1 \\
0 & \text{otherwise.}
\end{cases}
\end{align}

\subparagraph{Analysis}
By symmetry $\nabla_{\theta=0} \expect{x \sim p(\cdot|\theta)}{f(x)}=0$.
Take $n=2$ samples and define $x \equiv x^{(1)}$ and $z \equiv x^{(2)}$. The variance of the log-derivative estimator \eqref{eqn:logtrick:sum} at $\theta=0$ is then, defining $g_{\text{ld}}(x)\equiv f(x)\nabla_\theta \log p(x|\theta)$,
\begin{align}
\label{eqn:vld}
V_\mathrm{ld} 
& \equiv 
\expectlr{x,z\sim p(\cdot|\theta=0)}{\lnb \frac{1}{2}\big( g_{\text{ld}}(x) +g_{\text{ld}}(z)\big)\rnb^2 }
\\ & = \frac{12}{\pi }-\frac{15}{4}
\approx
0.0697.
\end{align}
The corresponding variance of our new estimator is, defining $g_\mathrm{ft}(x,z)=\frac{f'(z) \frac{1}{2} \sign (z-x)}{p(z|\theta)} \nabla_\theta \log p(x|\theta)$,
\begin{align}
V_\mathrm{ft} \equiv \expectlr{x,z\sim p(\cdot|\theta=0)}{\big( g_\mathrm{ft}(x,z)\big)^2}
 = \frac{4 \pi }{15}
\approx
0.838.
\end{align}
Although this is worse than $V_\mathrm{ld}$, the convex combination 
\begin{align}
& g_{\text{ld+ft}}(x,z,c)
\\ & ~~=
c \times \frac{1}{2}\big( g_{\text{ld}}(x) + g_{\text{ld}}(z)\big) + (1-c) \times g_\mathrm{ft}(x,z)
\end{align}
retains the correct expectation while enjoying a variance of
\begin{align}
V_\mathrm{ld+ft} 
& \equiv 
\expectlr{x,z\sim p(\cdot|\theta=0)}{\lnb g_\mathrm{ld+ft}(x,z,c)\rnb^2}
\\ & = 
\frac{4}{15} \pi  (c-1)^2+\frac{1}{4} c (53 c-68)+\frac{4 (40-31 c) c}{3 \pi }.
\end{align}
This is minimised at $c^\star=1-\frac{285 \pi -880}{\pi  (795+16 \pi )-2480}\approx 0.913$ obtaining a variance of (a closed form expression being available but messy)
\begin{align}
V_\mathrm{ld+ft}^\star \equiv \expectlr{x,z\sim p(\cdot|\theta=0)}{\lnb g_\mathrm{ld+ft}(x,z,c^\star)\rnb^2}
 \approx
0.898 \times V_\mathrm{ld},
\end{align}
where $V_\mathrm{ld}$ is the variance of the log-derivative estimator defined in \eqref{eqn:vld}.

\subparagraph{Discussion}

In this example, mixing an optimal $91.3\%$ of the log-derivative estimator with the remainder of our new estimator yields an $\approx 10.2\%$ improvement in the variance for $n=2$ Monte Carlo samples, with respect to the standard log-derivative estimator. 
The main point of the example is to demonstrate the general finding of \Autoref{sec:diversification}, namely that our new estimator includes an independent component of information with respect to the score function estimator, yielding lower variance in combination with it. 

\subparagraph{Baseline}

Finally, one typically includes a variance reducing baseline in the log-derivative estimator, replacing $g_\mathrm{ld}(x)$ with the still unbiased $g_{\text{ld+b}}(x,b)\equiv (f(x)-b)\nabla_\theta \log p(x|\theta)$ (the optimal variance reducing $b^\star$ of which may also be computed in closed form for this example). It is straightforward if somewhat messy to verify in a similar manner to the above that in that case, we retain a qualitatively similar although yet more modest improvement.


==> multidimensional.tex <==

\section{Multi-dimensional Fundamental Trick}
\label{sec:multid}

In one dimension we have exploited the fundamental theorem of calculus,
\begin{align}
f(x)-f(c)
& = 
\int_{z=c}^\infty \frac{\partial}{\partial z}f(z) \frac{\sign(x-z)}{2} \intd z.
\intertext{
More generally we have the gradient theorem
}
\label{eqn:gradienttheorem}
f(\bm x)-f(\bm c)
& = 
\int_{\bm z \in\gamma[\bm c, \bm x]} \nabla f (\bm z) \cdot 
\intd \bm z,
\end{align}
where $\gamma[\bm c, \bm x]$ is a path from $\bm c$ to $\bm x$.

\subsection{Linear path} 

Take $\gamma[\bm c, \bm x]$ to be the linear interpolation of 
$\bm 0 \rightarrow \bm x$, then from \eqref{eqn:gradienttheorem} we have 
\begin{align}
f(\bm x) - f(\bm c)
& = 
\int_{\bm z \in\gamma[\bm c, \bm x]} \nabla f (\bm z) \cdot 
\intd \bm z
\\
& = 
\int_{\alpha \in [0, 1]} \nabla f (\alpha \bm x + (1-\alpha) \bm c) \cdot 
(\bm x - \bm c) \intd \alpha,
\end{align}

\subsection{Sequential coordinate-wise} 

Take $\gamma[\bm 0, \bm x]$ to be the linear interpolation of the points 
\begin{align}
\bm 0 \rightarrow \mat{cccc}{x_1 & 0 & \cdots & 0}\ttran
\rightarrow \mat{ccccc}{x_1 & x_2 & 0 & \cdots & 0}\ttran\rightarrow \cdots \rightarrow \bm x
\end{align}
then from \eqref{eqn:gradienttheorem} we have 
\begin{align}
f(\bm x) - f(\bm 0)
& = 
\sum_{i=1}^d \int_{0}^{\infty} \frac{\sign(x_i-z_i)}{2} f^{(i)}\left(
\mat{cccccccc}{
x_1 & x_2 & \cdots & x_{i-1} & z_i & 0 & \cdots & 0
}\ttran
\right)
\intd z_i.
\end{align}

\subsection{Sequential partials}

Any of an increasingly higher order sequence of integral representations is valid:
\begin{align}
f(\bm x) - f(-\bm \infty) 
& =
\int_{-\infty}^\infty \frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccc}{z_1 & x_2 & \cdots & x_d}\ttran\rnb \intd z_1
\\
& =
\int_{-\infty}^\infty \frac{\sign(x_2-z_2)}{2} \partial_2 \int_{-\infty}^\infty \frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccccc}{z_1 & z_2 & & x_3 & \cdots & x_d}\ttran\rnb \intd z_1 \intd z_2
\\
& ~\, \vdots
\\
& = \int_{\realset^d}\prod_{j=1}^d \frac{\sign(x_j-z_j)}{2} \frac{\partial^d}{\prod_k \partial_k } f(\bm z) \intd \bm z.
\end{align}


Typically only a handful of derivatives will be non-vanishing. 

\subsubsection{$\partial_1$ non-vanishing only} 

In this case our estimator is 

\begin{align}
& 
\expectlr{\bm x \sim p(\cdot|\theta),z_1\sim \mathcal U
}{\frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccc}{z_1 & x_2 & \cdots & x_d}\ttran\rnb
\nabla_\theta \log p(\bm x | \theta)}
\\
& = 
\iint
p(\bm x|\theta)
\frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccc}{z_1 & x_2 & \cdots & x_d}\ttran\rnb
\nabla_\theta \log p(\bm x | \theta)
\intd \bm x \intd z_1
\\
& = 
\nabla_\theta
\iint
p(\bm x|\theta)
\frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccc}{z_1 & x_2 & \cdots & x_d}\ttran\rnb
\intd \bm x \intd z_1
\\
& = 
\nabla_\theta
\expect{\bm x\sim p(\cdot|\theta)}{
\int_{-\infty}^\infty 
\frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccc}{z_1 & x_2 & \cdots & x_d}\ttran\rnb \intd z_1
}
\\
& = 
\nabla_\theta
\expect{\bm x\sim p(\cdot|\theta)}{f(\bm x)-f(-\bm\infty)}
\\
\label{eqn:comical}
& = 
\nabla_\theta
\expect{\bm x\sim p(\cdot|\theta)}{f(\bm x)}.
\end{align}
But
\begin{align}
\hat\sigma_\mathrm{ll}
& = 
\expectlr{\bm x\sim p(\cdot|\theta)}{\big( f(\bm x)\nabla \log p(\bm x|\theta) \big)^2}
\shortintertext{and}
\hat\sigma_\mathrm{1l}
& = 
\expectlr{
\bm x\sim p(\cdot|\theta)
}{
\expectlr{z_1 \sim \mathcal U}{
\frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccc}{z_1 & x_2 & \cdots & x_d}\ttran\rnb
 \nabla \log p(\bm x|\theta) f(\bm x)\nabla \log p(\bm x|\theta) }}
\\
& = 
\expect{
\bm x\sim p(\cdot|\theta)
}{
f(\bm x)\big( \nabla \log p(\bm x|\theta) \big)^2\,\,
\smash{\underbrace{\expect{z_1\sim \mathcal U
}{
\frac{\sign(x_1-z_1)}{2} \partial_1 f \lnb\mat{cccc}{z_1 & x_2 & \cdots & x_d}\ttran\rnb
}
}_{= f(\bm x)}}
}
\\
& = 
\hat\sigma_\mathrm{ll}.
\end{align}



==> vae_example.tex <==

\subsection{Variational Autoencoder Example}
\label{sec:experiments:vae}

\subparagraph{Setup} We trained a variational autoencoder (VAE) \citep{vae} on the MNIST dataset. Rather than use the reparameterisation trick (which is applicable for a Gaussian approximate posterior), for the purpose of demonstration we use the log-derivative trick and the representer trick. We used a typical computational setup with a 5 latent dimensions and 400 hidden units.

\subparagraph{Experiment} The evidence lower bound (ELBO) objective as optimised by the VAE decomposes into a tractable regularisation term and an intractable expected log likelihood term which requires stochastic approximation. We experimented with different estimators of the (gradient of) the expected log-likelihood, for consumption by a standard numerical optimiser. We mixed various fixed proportions $c$ of our new representer trick estimator with $(1-c)$ of the log-derivative estimator. The smoothing parameter $a$ of \Autoref{sec:multivariate} was set to $1$ (to be on the same range as the prior variance of the latent encoding, which was also $1$) and applied the multivariate representation of \sref{Lemma}{lem:multivariate:noncompact} with a first order approximation, \textit{i.e.} retaining up to first order derivatives (in the notation of \citep{vae} these derivatives are $\nabla_{\bm z} \log p_{\bm \theta}(\bm x^{(i)} | \bm z)$, evaluated at a sample from the approximate posterior $\bm z \sim q_{\bm \phi}(\bm z|\bm x^{(i)})$).

\subparagraph{Results and Discussion} The training curves of \Autoref{fig:vae} show that mixing 20\% of the new estimator yields an improvement in the loss of around 7\%. This demonstrates that under more realistic scenarios than the toy example of \Autoref{sec:experiments:analytical}, our new family of estimators does offer a relevant source of new information in comparison with the log-derivative trick. %
Note that the linear combination employed here is very simplistic, and while the improvement demonstrated here is modest,  we conjecture that more refined approaches exist with stronger performance --- \textit{examples:} adaptive choice of and/or averaging over of the Sobolev length-scale parameter $a$; robust combination of the $n(n-1)$ terms summed in \eqref{eqn:pairwisevariance:mn}; adaptive/robust combination of the representer trick with the log derivative trick, \textit{etc}. However, such developments are rather non-trivial, and beyond the present scope. %

